An Empirical Study on Content Bundling in BitTorrent Swarming System

Despite the tremendous success of BitTorrent, its swarming system suffers from a fundamental limitation: lower or no availability of unpopular contents. Recently, Menasche et al. has shown that bundling is a promising solution to mitigate this availability problem; it improves the availability and reduces download times for unpopular contents by combining multiple files into a single swarm. There also have been studies on bundling strategies and performance issues in bundled swarms. In spite of the recent surge of interest in the benefits of and strategies for bundling, there are still little empirical grounding for understanding, describing, and modeling it. This is the first empirical study that measures and analyzes how prevalent contents bundling is in BitTorrent and how peers access the bundled contents, in comparison to the other non-bundled (i.e., single-filed) ones. To our surprise, we found that around 70% of BitTorrent swarms contain multiple files, which indicate that bundling has become widespread for contents sharing. We also show that the amount of bytes shared in bundled swarms is estimated to be around 85% out of all the BitTorrent contents logged in our datasets. Inspired from our findings, we raise and discuss three important research questions in the field of file sharing systems as well as future contents-oriented networking: i) bundling strategies, ii) bundling-aware sharing systems in BitTorrent, and iii) implications on content-oriented networking.

==> conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

Content availability is a serious problem in today's peer-to-peer
swarming systems. Menasche \textit{et al.} has shown that bundling
is a promising solution to mitigate this availability problem, but
there are still little empirical grounding for understanding,
describing and modeling it. This is the first empirical study that
measure and analyze how prevalent contents bundling is in BitTorrent
and how peers access the bundled contents, in comparison to the
single-filed ones. To our surprise, we found that bundling has
become widespread for contents sharing. Inspired from our findings,
we raise and discuss three important research questions in the field
of file sharing techniques/architecture as well as future
contents-oriented networking: i) bundling strategies, ii)
bundling-aware sharing systems in BitTorrent, and iii) implications
on content-oriented networking.


==> introduction.tex <==
\section{Introduction} \label{sec:introduction}

% BitTorrent success
BitTorrent~\cite{BitTorrent} has become the de facto standard in
sharing contents on the Internet. According to the Ipoque's report
released in 2009~\cite{Ipoque2009}, BitTorrent accounts for
approximately 27-55\% of today's Internet traffic. The ever
increasing usage of BitTorrent is attributed to some attractive
properties of its swarming systems: First, cooperation among peers
in a swarm stimulated by the tit-for-tat based incentive mechanism
to improve the overall system performance in terms of throughput.
Second, the tit-for-tat strategy also prevents (or mitigates) the
free-riding problem. Third, the swarming technique scales well even
in the presence of massive flash crowds for popular
contents~\cite{SIGMETIRC07, NSDI07}.

% Bundling in BitTorrent
Despite the success of BitTorrent, its swarming system suffers from
a fundamental limitation: little or no availability of unpopular
contents. That is, peers arriving after the initial flash crowd may
often end up with finding the content unavailable, not to mention
unpopular contents~\cite{CoNEXT2009}. Recently, Menasche \textit{et
al.} has shown that \emph{bundling} is a promising solution to
mitigate this availability problem; it improves the availability and
reduces download times for unpopular contents by combining multiple
files into a single swarm~\cite{CoNEXT2009}. There also have been
studies on bundling strategies~\cite{GAMENET2009, INFO2010} and
performance issues in bundled swarms~\cite{ICCP2006}.

In spite of the recent surge of interest in the benefits of and
strategies for bundling, there is still little empirical grounding
for understanding, describing, and modeling it. This leaves
researchers uncertain of (i) whether and how the assumptions (on
both bundling pattern and user access pattern~\cite{CoNEXT2009,
ICCP2006}, with little if any empirical evidence) made in the
aforementioned work are congruent with (or close to) reality, and
(ii) the status quo and performance and architectural implications
of bundling for the advancement of file sharing techniques or
architectures (not to mention BitTorrent), as well as of the
so-called future \emph{`content-oriented networking'}.

% contributions
To begin to provide empirical grounds for understanding, describing,
and modeling contents bundling in BitTorrent, we make the following
contributions: (1) This is the first empirical study that measures
and analyzes how prevalent contents bundling is in BitTorrent and
how peers access the bundled contents, in comparison to the other
non-bundled (i.e., single-filed) ones. To this end, we first
developed a BitTorrent monitoring software by modifying the
Azureus~\footnote{Azureus is also called Vuze, one of the most
popular BitTorrent client.}~\cite{vuze}, one the most popular
BitTorrent clients. Using the developed code, we have collected over
a month of data comprised of 36K distinct swarms of 2.8 Million
distinct peers. (2) To our surprise, we found that around 70\% of
BitTorrent swarms contain multiple files, which indicate that
bundling has become widely used for contents sharing. (3) We also
estimated that the amount of bytes shared in bundled swarms are
larger than that in single-filed swarms: The amount of data
contained in bundled swarms are about 2 times larger than
single-filed ones, the number of bundled swarms are about 2.3 times
in average larger than that of single-filed ones, and the average
popularity of bundled swarms are 1.2 times larger than single-filed
ones, which we approximately estimate that amount of bytes shared in
bundled contents account for around 85\% out of all the BitTorrent
contents logged in our datasets. (4) According to our measurements,
the bundling pattern and user access pattern are different depending
on the seven BitTorrent content type categories (i.e., Movie, Porn,
TV, Music, Applications, E-book, and Game). (5) Based on our
findings and lessons learned, we raise and discuss three new
important research questions in the area of file sharing systems as
well as the future contents-oriented networking: i) bundling
strategy, ii) bundling-aware swarming systems in BitTorrent, and
iii) implications on content-oriented networking.

% paper organization.
This paper is organized as follows. After reviewing related work in
Section~\ref{sec:related}, we present measurement methodology, data,
and results in Section~\ref{sec:measurement}.
Section~\ref{sec:ongoing} discusses on implications of content
bundling and our ongoing work. Finally, we conclude this paper in
Section~\ref{sec:conclusion}.


==> related.tex <==
\section{Related Work}\label{sec:related}

% BitTorrent and swarming systems
\textbf{BitTorrent:} BitTorrent~\cite{BitTorrent} has been the de
facto standard for content sharing. Due to its success in the real
world, many studies have been conducted to investigate BitTorrent's
behavior in terms of throughput, fairness and incentive issues,
revealing valuable insights into the performance aspect of the
BitTorrent~\cite{FairTorrent, NSDI07, SIGCOMM04, SIGMETIRC07}.

% Multi-torrent.
\textbf{Sharing Multiple Files:} Most studies on BitTorrent had
focused only on sharing and transmission of single torrents until
Guo \textit{et al.} found that 85\% of users concurrently access
multiple torrents~\cite{IMC2005}. Yang \textit{et
al.}~\cite{MASCOTS2008} proposed a novel incentive mechanism for
remaining as seeds in a subset of downloaded torrents when a user
downloads multiple torrents. This mechanism calculates the
aggregated downloading rate in a \emph{cross-torrent} fashion in the
peer selection phase, so that a node can get additional credits from
providing pieces in another torrent which it participates in as a
seed. These studies assume that only a single file is shared in a
single swarm. In contrast, we focus on ``bundling'', which allows
peers to download multiple files from a single swarm.

% Bundling
\textbf{Bundling:} Recently, Menasche \textit{et
al.}~\cite{CoNEXT2009, GAMENET2009} has shown that bundling can
mitigate the availability problem by combining multiple files into a
single swarm. Also Tien \textit{et al.} studied the performance
issues in sharing multiple files not only using multiple torrents
but also using a bundle in BitTorrent~\cite{ICCP2006}. Despite the
recent surge of interest in the benefits of and strategies for
bundling, there are still little empirical grounding for
understanding, describing, and modeling it.

